Jut: A Framework for Just-in-Time Data Access

With the proliferation of sensor and personal devices, our physical spaces are now awash in potential data sources. In principle this data could serve a wide range of applications and services. However, leveraging these data sources is challenging with today's systems because they are not typically designed to consume data opportunistically, from a new device that happens to arrive in the vicinity. In this paper, we present the design and implementation of Jut, a system designed for "Just-in-Time" data access - in which an application is able to discover and consume data from any available source, even ones not known at development or installation time. Jut combines two novel design choices: modularizing data processing systems to better reflect the physical world, and a new form of application-data integration that equips data processing pipelines with the information they need to process new and evolving data formats and schemas. We show that these choices greatly simplify the development and use of smart-space and IoT applications. For a representative set of devices and application scenarios, we show that Jut can implement use-cases not easily supported today, or can do so with 3.2-14.8x less development effort and 3-12x lower query complexity than current systems.

==> design.tex <==
\section{\arch Design}
\label{sec:design}

This section presents the design of \arch framework. 

\subsection{Design Rationale}



\subsection{Context Data Router}
\label{subsec:abs}

\begin{figure}
     \centering
     \footnotesize
     \includegraphics[width = 0.43\textwidth]{dia/router.pdf}
     \caption{\textbf{Context data router (\cdr) abstraction.} $R.ig$: ingress pipelet. $R.eg$: egress pipelet. $R.store$: context data store.}
     \label{fig:router}
     \figspace
\end{figure}

%

%

%

\pb{Context data store, $R.store$.} The store is an append-only, persistent data storage that stores data as an ordered list of data records in Zed binary format~\cite{zng}, where data records are self-describing and hence no predefined schemas are required for ingesting new data and heterogeneous data can co-exist. While not strictly necessary, we chose to build \arch using Zed since it offers a convenient way to ingest and represent eclectic data (\S\ref{sec:related}). The store exposes a data \texttt{load()} interface that the data ingresses of the \cdr can write new data records to, as well as a \texttt{query()} and a \texttt{watch()} API that the egresses can read data from, which we describe next.

\pb{Ingress pipelet, $R.ig$.}  An ingress of a \cdr pulls data from one or multiple data sources specified in $ig.sources$, a process we'll describe in \S\ref{subsec:cdf}. A \cdr can have multiple ingresses, each identified by $ig.id$. Each ingress processes the ingested data with its dataflow ($ig.flow$), which contains operators (\eg sort, join) and functions (\eg sum, avg) that process a sequence of input data records from $ig.sources$ and generate a sequence of output records. The resultant \emph{derived} data is written to $R.store$.  $R.ig$ has two methods of ingesting data: \emph{native} or \emph{proxied} ingestion. In native ingestion, $R.ig$ ingests data directly from other \cdrs' egresses (described next). On the other hand, proxied ingestion involves a \emph{proxy} accessing data from the device through a device communication library like the Matter protocol~\cite{matter} or via the device vendor cloud. In this paper, we assume the setup where data from a device is first ingested into a \emph{device \cdr} through proxied ingestion, and other \cdrs subsequently access the data from the device \cdr via native ingestion. %

\pb{Egress pipelet and view, $R.eg$.} An egress exposes data records in $R.store$ to data consumers such as other \cdrs, apps, and users. $R.eg$ can also be associated with a dataflow. At run-time, $R.eg$ reads from $R.store$, processes the data with $eg.flow$, and then caches it persistently; and we refer to this resultant data as the \emph{egress view}, borrowing the notion of views from databases~\cite{noria,risingwave,postgres}. The egress supports a \texttt{query()} and a \texttt{watch()} interface to read records from its view (similar to $R.store$). The \texttt{query()} interface allows one to query against the egress as a list of records, while \texttt{watch()} allows one to subscribe to the egress as an unbounded stream of data records. A \cdr can have multiple egresses, each identified by $eg.id$, and any entity (app or another \cdr) can retrieve data about a context by querying one or more of its \cdr's egresses. Finally, $eg.schemas$ stores the schemas of the data records in the egress view, while $eg.policy$ is used for specifying access control policies over these records, which we'll discuss in detail in \S\ref{subsec:cdf} and \S\ref{subsec:security} respectively.

\begin{table}[]
\footnotesize
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Name} & \textbf{Notation} & \textbf{API} & \textbf{Description} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Data\\ Store\end{tabular}} & \multirow{2}{*}{$R.store$} & load() & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Store context data as \\ an ordered list of records\end{tabular}} \\ \cline{3-3}
 &  & query() &  \\ \hline
\multirow{5}{*}{Ingress} & \multirow{5}{*}{$R.ig$} & .id & \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Pull, process, and load data \\ to $R.store$ from data sources,\\ which can be specified as intents\\ that get resolved at run-time\end{tabular}} \\ \cline{3-3}
 &  & .intent &  \\ \cline{3-3}
 &  & .sources &  \\ \cline{3-3}
 &  & .policy&  \\ \cline{3-3}
 &  & .flow &  \\ \hline
\multirow{5}{*}{Egress} & \multirow{5}{*}{$R.eg$} & .id & \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Process and expose data \\ in $R.store$ to data consumers\\ while enforcing access policy\end{tabular}} \\ \cline{3-3}
 &  & .flow &  \\ \cline{3-3}
 &  & .schemas &  \\ \cline{3-3}
 &  & .policy &  \\ \cline{3-3}
 &  & .query() &  \\ \hline
\multirow{3}{*}{Metadata} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}$R.meta$\\ (or $R$)\end{tabular}} & .kind & Kind of the CDR \\ \cline{3-4} 
 &  & .name & Name of the CDR instance \\ \cline{3-4} 
 &  & .role & Role assigned for access control \\ \hline
\end{tabular}
\caption{Main components and their APIs in the \cdr.}
\label{tab:abs}
\figspace
\figspace
\end{table}

\pb{\cdr kind.} A \cdr includes three metadata pieces: \emph{kind} ($R.kind$), \emph{name} ($R.name$), and \emph{role} ($R.role$). Developers can create new types of \cdrs identified by $R.kind$, such as the \texttt{cot.dev/v1/Building} in Fig.\ref{code:building} . %

The rationale behind the approach of having \cdr kind is that while there are many devices/contexts, there are relatively fewer device/context kinds that will be of interest to a specific \cdr. Developers can write data processing pipelines  for these kinds, and this approach encourages a natural consolidation towards a few popular/canonical or standard kinds (\eg apple.com/v1/iphone) while still allowing flexibility to support more niche kinds (vendor\_x/v1/phone) and evolve the supported kinds over time (vendor\_x/v2/phone). Another benefit of \cdr kind is that developers can indicate ingesting data from \cdr kinds rather than specific \cdrs as the latter might not be always known at the development time (\S\ref{subsec:cdf}). We explain $R.role$ for access control in \S\ref{subsec:security}.

%

Table~\ref{tab:abs} summarizes the \cdr abstractions, and further details on \cdr programming will be discussed in \S\ref{sec:prog}.

\subsection{Contextualized Dataflow Graph}
\label{subsec:cdf}

In \arch, \cdrs can be composed into a data flow graph called the \emph{contextualized dataflow graph} (CDG), which allows data to flow from one \cdr's egress to another's ingress. The CDG is formed and continuously updated to reflect changes in context associations resulting from join and leave operations. The main challenge is that \cdr developers may not know in advance at development time which data sources---their names, kinds, or the schemas of their data records---the \cdr should ingest from at any given time, as data sources may only appear opportunistically in a context. For instance, data from Alice's phone may only be available in a room when Alice is present and has opted to share her data. \arch provides two mechanisms, \emph{context-based sourcing} and \emph{schema reconciliation}, to address these challenges.

\pb{Context-based sourcing.} The developers of a \cdr X define what data sources a particular ingress pipelet $X.ig$ can ingest and process in $X.ig.intent$. The sourcing intent can be a \emph{direct} reference in the form of $cdr@egress$, where $cdr$ is the name of the \cdr and $egress$ is the name of its egress. This is used when the specific data source is known at development time, such as ingesting weather updates from a public weather API. Alternatively, the sourcing intent can be an \emph{indirect} reference to data sources that can only be determined at runtime, in the form of $kind@egress$, where $kind$ refers to all \cdrs under the $kind$, and $egress$ is an egress's ID. Wildcards for \cdr kind like $any@egress$ is also supported as described next.

\begin{algorithm}
\caption*{\textbf{Algorithm 1:} Contextualized Dataflow Graph Composition}
\label{algo:join}
\begin{algorithmic}[1]
\State \textbf{Input:} Context $X$ and $Y$
\Procedure{OnJoin}{$Y$, $X$}
    \For{\textbf{each} ingress $i$ \textbf{in} $X.ig$}
        \For{\textbf{each} sourcing intent $s$ \textbf{in} $i.intent$}
            \If{not match($s.kind$, $Y.kind$)}
                \State \textbf{continue}
            \EndIf
            \For{\textbf{each} egress $e$ \textbf{in} $Y.eg$}
                \State \textbf{if} ($e.id == s.egress$ \textbf{\&\&}
                \State \hspace{\algorithmicindent}allow($e.policy$, $X.role$)) \textbf{then}
                    \State \hspace{\algorithmicindent}$i.flow$.inject($e.schemas$, $i.policy$)
                    \State \hspace{\algorithmicindent}$i.sources$.append($e$)
            \EndFor
        \EndFor
        \State $i$.restart\_if\_changed($i.sources$, $i.flow$)
    \EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}

At run-time, \arch resolves the sourcing intent in $X.ig.intent$ based on the available sources in the context and including them in the $X.ig.sources$. Algorithm 1 describes this CDG composition process when a context join occurs.  At a high level, when a context Y joins X, \arch performs the following steps: \textbf{(i)} Matching the kind and egress specified in the sourcing intent to Y's kind and egresses, where developers of context X can define matching policy for kind matches. Common matching forms include exact matches on group, version, and kind name (denoted as g/v/n), wildcards on version (g/*/n), wildcards on both group and version (*/*/n), and using the ``any'' keyword as a wildcard for kind. \textbf{(ii)} Filtering the resultant egresses based on the access control policies (\S\ref{subsec:security}); \textbf{(iii)} Updating the $ig.sources$ (and $ig.flow$ based on the schema reconciliation policy, described next), and finally \textbf{(iv)} reconfiguring X's ingress if any of its sources change. Besides, when a leave(Y, X) operation occurs, \arch removes all of Y's egresses from the $X.ig.sources$. With the context-based sourcing, \arch ensures that the CDG remains up-to-date according to context associations and thus enables a \cdr to \emph{opportunistically} ingest data from other \cdrs in the context to which it has sufficient access. %

Fig.\ref{fig:sourcing} illustrates opportunistic data ingestion with \arch. In this example, a phone \cdr with an egress named/ID-ed $noise$ moves between rooms, and the room \cdrs include the $any@noise$ sourcing intent in their $ig.intent$ to ingest noise measurements from the phone. The source resolution occurs whenever there is a change in the context association in the control plane, and this coordination is automated by \arch's coupler abstraction, which we'll describe in \S\ref{subsec:control}.
%

\begin{figure}
     \centering
     \footnotesize
     \includegraphics[width = 0.48\textwidth]{dia/sourcing.pdf}
     \caption{\textbf{Opportunistic ingestion.} As a phone moves from Room A to B (left), \arch ensures each room's \cdr correctly ingests data streams from the phone's \cdr by resolving the sourcing intent dynamically according to the control plane join/leave events (right).}
     \figspace
     \label{fig:sourcing}
\end{figure}

 %

%
\[
\begin{tabular}{ll}
\textbf{Match} & \textbf{Action} \\
\text{has <watt: string>} & \text{extract} \\
\text{has <power: string>} & \text{rename watt:=power} \\
* & \text{reject} \\
\end{tabular}
\]

%

%

%


\subsection{\arch Control Plane and Coupler}
\label{subsec:control}

The control plane in \arch is responsible for storing \cdr metadata, context associations, and user policies, and it provides the \cc abstraction for control logic. Similar to other frameworks~\cite{dspace}, \ccs in \arch's control plane can be organized into a control hierarchy that reflects the context associations (\eg lamp to room and room to building). This allows a child \cc to be joined to a parent \cc using the join/leave API, enabling the parent to send control messages to instruct the child's behavior. Since both the control and data planes contain abstractions for contexts (\ie context associations, join/leave, \cc, and \cc hierarchy; \cdr and CDG), they need to be coordinated to ensure proper functioning of apps.

\pb{Cross-plane coordination.} First, ensuring that the CDG's source resolution accurately reflects context associations requires \emph{coordination} between \arch's control and data planes. Cross-plane coordination is also required when developing apps that involve both control and data functionalities. For instance, to implement a control app that alerts of overcrowding or abnormalities based on occupancy data, there should be a room \cc in the control plane that implements the actuation logic and a corresponding room \cdr in the data plane that stores the occupancy data. The room \cc can query its corresponding \cdr for occupancy data to implement the alerting logic. However, such coordination can be tedious and error-prone if developers are responsible for implementing them on a per-app basis, which is typically the case in existing frameworks where the two planes are integrated only in a bespoke manner. 

\pb{Coupler.} To address this, \arch provides an explicit coupling between the control and data planes through the \emph{coupler} abstraction, which automates the control-data plane coordination. To support the CDG, the coupler in \arch watches for changes in the control plane related to context associations. . To support control apps, when a context has both a \cc and a \cdr, the coupler enforces a 1:1 mapping between the \cc and its corresponding \cdr for that same context. This means that every time the control plane creates, deletes, or updates a \cc, the coupler correspondingly creates, deletes, or updates the \cdr for that context. The \cc can access its \cdr data (with APIs in \S\ref{sec:prog}) without the need to explicitly discovering the \cdr. Further, the coupler reconfigures the \ccs so that they and the \cdrs act in accordance with context association updates. For example, when \texttt{join(lamp, room)} is invoked in \arch, the coupler also reconfigures the room's \cc to allow it to observe and control the lamp's power and intensity levels. At the same time, \arch resolves the source intent and reconfigures the room \cdr's ingress, enabling the \cdr to consume the lamp's energy readings.

\subsection{Context Data Policy and Security}
\label{subsec:security}

There is an extensive literature on system support~\cite{secure-iot-gw, iotguard, lofti, dspace, capture} and user expectations~\cite{nick-user, franzi-user, franzi-multiuser} for data privacy and security in mobile and IoT applications. This literature identifies four essential goals: data ownership, access control, provenance, and governance, and presents various techniques to achieve them. Pertinent to \arch's design is how to realize these techniques for \emph{context data}. We elaborate on this in what follows.

\pb{Access control.} Data records in \cdrs are accessible via the egresses. \arch leverages Role-based Access Control (RBAC) to dictate which \emph{role} can access which egress, and \arch's first-class context abstraction allows for the association of such roles with the \cdrs ($R.role$). \arch maintains Access Control Lists (ACLs) for each role. These ACLs are based on the access policies specified by users in the form of allowlists or blocklists associated with each egress ($R.eg.policy$). Users can specify these egress policies during \cdr creation and can update them at run-time such as during \cdr registration. \arch's source resolution only resolves those egresses that a \cdr has been granted access to. For example, when Alice grants only BioLab access to her Phone's ``location'' egress, only the BioLab is able to ingest data when the phone joins but not PhyLab. 

\pb{Ownership.} \arch enables each \cdr operator to maintain control over what context data is stored and where. To better support this, \arch allows for the separation of data tenancy, storing data for different contexts in different \cdrs. Each \cdr can further choose the storage system it wants for its data store, and as we implement \cdr as a microservice (\S\ref{subsec:runtime}), it can be deployed and operated independently on separate compute and storage infrastructure.

\pb{Provenance and governance.} A \cdr can be used to support data provenance by tracking the sources of ingested data (\eg the names of the \cdrs and egresses that an ingress ingests data from) and operations that generate or modify the data (\eg data loaded by \cc). This information is stored either with the data records or their associated metadata (\S\ref{sec:prog}). For instance, as shown in Fig.\ref{code:building} (L16) and Fig.\ref{fig:building-records} (last two records), when the \texttt{patch\_from} option is enabled in the ingress configuration, the \cdr will add a \texttt{from: source@egress} field to the data. This ``from'' can also be a sorted array that tracks the \cdrs the record is generated along the path (\eg \texttt{from: [BioHall@occupancy, BioLab@occupancy, desk@detected]}) as a lineage. 



==> eval.tex <==
\section{Evaluation}
\label{sec:eval}

We evaluate \arch to answer the following questions:

\squishlist
\item How does \arch simplify the \emph{use} and \emph{development} of JIT-DA apps in smart spaces, compared to existing frameworks? (\S\ref{subsec:result} and \S\ref{subsec:benefit})
\item What are the contributions of the design choices in \arch towards its \emph{benefits} in app development and use? (\S\ref{subsec:benefit})
\item What are the \emph{performance} implications of \arch's designs, and is our implementation performant enough to meet real-world requirements? (\S\ref{subsec:benchmark})
\squishend

\noindent We start by describing the apps (\S\ref{subsec:app}) and setup (\S\ref{subsec:setup}).


\subsection{Example Applications}
\label{subsec:app}

We select 5 representative apps and 7 common app scenarios (denoted S1-S7) across them: smart campus (S1-S2), urban sensing (S3-S4), supply chain analytics (S5), smart home (S6), and personal carbon footprint (S7), each emphasizing a set of requirements and challenges which we highlight inline. 

\pb{(1) Smart Campus.} A smart campus~\cite{cisco-campus,stanford-campus,deloitte-campus} leverages mobile and IoT/smart space technologies to optimize campus operations and improve the experience for students, faculty, and staff on university or company campuses. It enables data-driven insights and decision-making to reduce energy costs, optimize resource utilization, and provide real-time information and personalized services for tenants. We highlight two representative apps in smart campus: space analytics~\cite{venturebeat,density,comfy}, which tracks occupancy for contexts and optimizes their utilization; and energy monitoring~\cite{smart-building,mortar}, which estimates energy consumption for contexts such as rooms and buildings. Specifically, in our first scenario, \underline{{\bf S1}}, we focus on supporting \emph{query over contexts}: we want to query rooms for their energy usage and occupancy, identify the rooms that are least occupied or most energy-consuming, while also analyzing the correlation between energy usage and occupancy. Meanwhile, we also aim to \emph{reuse context data} or reuse \emph{contexts as data sources} when developing new apps. For example, in \underline{\textbf{S2}}, we want to enable building-level energy and occupancy estimation by reusing data from rooms.

\pb{(2) Urban Sensing.} Urban sensing~\cite{citizen-science,mit-sense,burke2006participatory,streetlight} collects and analyzes data about urban environments, such as network quality, noise levels, air pollution, and so on, using inexpensive or crowdsourced sensors, as well as more traditional sensors and devices. In \underline{{\bf S3}}, we aim to leverage urban sensing to enhance the smart campus experience by allowing people to identify rooms with both good network and low occupancy. To achieve this, we want to allow \emph{opportunistic ingestion} of network quality data from tenants' laptops and smartphones. Besides, we need to restrict data access over contexts in the smart campus. Thus in \underline{{\bf S4}}, we aim to specify policies that restrict students' access to data on network quality and occupancy (not energy usage) and lab rooms (not faculty offices). %

\pb{(3) Supply Chain Analytics.} Supply chain analytics~\cite{cargosense,samsara,afresh,souza2014supply} uses data analytics to extract insights from supply chain data and improve overall supply chain performance, visibility, and control. In \underline{{\bf S5}}, we focus on analyzing the cargo shipment delays across ports and warehouses while respecting the \emph{distributed control} of these supply chain nodes. This means that the cargo information is stored independently at each node, and the app should query each node to gain a complete understanding of the shipment delays.

\pb{(4) Home Automation.} Home automation, or smart home~\cite{homeassistant,smartthings,dspace,matter,bolt,mare2019consumer}, is a popular application in IoT that controls and automates household functions, such as lighting, temperature, security, and entertainment. In \underline{{\bf S6}}, we aim to implement \emph{data-driven automation} for 1. Automatically setting the brightness levels of a room's lamps based on its past average brightness settings when the room's door is opened; and 2. Security and overcrowding detection by sending an SMS message to the home owner based on room occupancy. To enable these automations, we need to allow the smart home's actuation logic to easily access/query context data.

\pb{(5) Personal Carbon Footprint.} A Personal Carbon Footprint app enables individuals to track their carbon emissions from daily activities and identify opportunities to reduce their environmental footprint~\cite{carbon-app,carbon-calculator,carbon-pricing}. In \underline{{\bf S7}}, we aim to implement an app for the smart campus that allows tenants to track their energy consumption at different locations on campus during their stay. To achieve this, the app must be able to \emph{opportunistically consume data} from different contexts and handle \emph{heterogeneous data}, such as energy readings with unexpected schemas, across these contexts.

\subsection{Experiment Setup}
\label{subsec:setup}

We describe our testbed and experiment setup as follows.

\begin{table}
\footnotesize
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Device} & \textbf{Brand} & \textbf{Model} & \textbf{Native API} & \textbf{QTY} \\ \hline
Smartphone & Apple & iPhone 13 Pro Max & Jut client & 2 \\ \hline
Laptop & Apple & Macbook Air M1 & Jut client & 2 \\ \hline
\begin{tabular}[c]{@{}c@{}}Underdesk \\ PIR\end{tabular} & Pressac & \begin{tabular}[c]{@{}c@{}}Wireless desk \\ motion detector\end{tabular} & \begin{tabular}[c]{@{}c@{}}Pressac \\ cloud\end{tabular} & 2 \\ \hline
Motion & Ring & Alarm Security Kit & Ring-client & 6 \\ \hline
\begin{tabular}[c]{@{}c@{}}Contact \\ Sensor\end{tabular} & Eve & Door \& Window & Matter & 4 \\ \hline
Heater+Fan & Dyson & HP01 & Dorita980 & 1 \\ \hline
Plug & Eve & \begin{tabular}[c]{@{}c@{}}Plug \& Power \\ Meter\end{tabular} & Matter & 4 \\ \hline
\begin{tabular}[c]{@{}c@{}}Smart light \\ bulb\end{tabular} & Lifx & Mini & Lifxlan & 8 \\ \hline
\end{tabular}
\caption{Devices in our testbed.}
\label{tab:device}
\figspace
\end{table}

\pb{Devices.} We use real-world devices to implement the apps above (except for S5, which we simulate with contexts). Table~\ref{tab:device} summarizes the physical devices used in the experiments. Two types of detectors, Pressac~\cite{pressac} and Ring~\cite{ring-motion}, are used to detect occupancy by signaling whether there is motion or not. Smart light bulbs, Lifx~\cite{lifx-light}, are used as lamps; Dyson~\cite{dyson} heater and Eve plugs~\cite{eve-plug} that are connected to electrical appliances, \eg TV, fridge, air purifier; contact sensors~\cite{eve-door} are used to detect door open/close. Finally, Apple laptops and smartphones are used as devices that both contribute data to contexts as well as run user-facing apps that consume data from contexts.

\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Context} & \textbf{Symbol} & \textbf{Ingress} & \textbf{Egress} \\ \hline
Motion & $M$ & Native API & detected \\ \hline
Lamp & $L$ & Native API & \begin{tabular}[c]{@{}c@{}}energy, \\ brightness\end{tabular} \\ \hline
Appliance & $A$ & Native API & energy \\ \hline
Room & $R$ & \begin{tabular}[c]{@{}c@{}}Motion.detected, \\ Smartphone.conn, \\ *.energy\end{tabular} & \begin{tabular}[c]{@{}c@{}}netSpeed\\ energy\\ occupancy\end{tabular} \\ \hline
\begin{tabular}[c]{@{}c@{}}Building, Floor,\\ Department\end{tabular} & $B$, $F$, $D$ & \begin{tabular}[c]{@{}c@{}}Room.energy, \\ Room.occupancy\end{tabular} & \begin{tabular}[c]{@{}c@{}}energy, \\ occupancy\end{tabular} \\ \hline
Campus & $C$ & \begin{tabular}[c]{@{}c@{}}Building.energy, \\ Building.occupancy\end{tabular} & \begin{tabular}[c]{@{}c@{}}energy, \\ occupancy\end{tabular} \\ \hline
\begin{tabular}[c]{@{}c@{}}Smartphone,\\ Laptop\end{tabular} & $P$ & \begin{tabular}[c]{@{}c@{}}Smartphone, \\ *.energy\end{tabular} & \begin{tabular}[c]{@{}c@{}}conn, \\ bssid\end{tabular} \\ \hline
Port, Airport & $Po$, $Ao$ & *.cargo & delay \\ \hline
Ship, Plane & $S$, $J$ & - & cargo \\ \hline
\end{tabular}
\caption{Kinds of contexts used in the experiments.}
\label{tab:setup}
\figspace
\end{table}

\pb{Contexts.} Table~\ref{tab:setup} describes the contexts and their contexts implemented for S1-S7 using \arch, including the data sources they pull data from (\eg a Room context pulls data from an Motion's @detected) and the egresses they expose. For smart campus and urban sensing (S1-S4), we installed the devices in 4 rooms/offices, where each room has one contact sensor, two motion detectors, two lamps, and one appliance; Fig.\ref{fig:scenario}a depicts how the contexts are organized according to the context associations. Each room also has its own WiFi access point (AP). The room setup is reused for the home automation (S6) and carbon footprint tracking (S7). For supply chain (S5), we simulate the contexts (\eg ships and ports) with synthetic data and events. Unless otherwise mentioned, we run the software components (\arch runtime, Zed lake, dSpace, and the baselines) using Kubernetes (v1.21.0) in a Thinkcentre M720 machine (Intel Core i5-8400T, 6 cores).

\begin{figure}[t]
     \centering
     \footnotesize
     \includegraphics[width = 0.46\textwidth]{dia/scenario.pdf}
     \figspace
     \caption{Visualization for devices and contexts in S1-S7. The notations for the contexts can be found in Table~\ref{tab:setup}.}
     \label{fig:scenario}
     \figspace
\end{figure}

\pb{Baselines.} We compare \arch to two app frameworks: AWS IoT~\cite{aws-iot} with AWS Timestream~\cite{aws-timestream} for data processing and dSpace~\cite{dspace} with Postgres~\cite{postgres}. AWS IoT is widely used in industry, while dSpace and Postgres are representative of the latest progress in academia and open-source communities. These frameworks were used to implement the app scenarios, and the one best suited for each scenario was selected due to missing support for features across all frameworks.

\pb{Metrics.} Our metrics for evaluating the \emph{ease-of-development} and \emph{ease-of-use} of the JIT-DA apps and scenarios are the \emph{development effort} and \emph{query complexity}, respectively.

\noindent {\it 1. Development effort: SLOC.} To measure the ease of development, we count the source lines of code, configurations, and scripts required to build and support an app.

\noindent {\it 2. Query complexity: Qcx.} We use query complexity (Qcx) to estimate the effort required to write queries against context data. Qcx is calculated by summing the number of dataflow operators and data subjects in a query. For example, a query with two data subjects and one dataflow operator, such as \texttt{BioHall@occupancy "avg()"}, has a Qcx of 3.\footnote{We recognize that there is no widely accepted method for measuring query complexity, and hence we adopt this simple approach, inspired by what's studied in prior literature~\cite{software-complexity,sql-complexity}.} 

\subsection{Implementing S1-S7 with \arch}
\label{subsec:result}

\begin{table*}[]
\centering
\footnotesize
\begin{tabular}{|c|cccc|c|c|c|}
\hline
\textbf{App:} & \multicolumn{2}{c|}{\textbf{Smart Campus}} & \multicolumn{2}{c|}{\textbf{Urban Sensing}} & \textbf{Supply Chain} & \textbf{Smart Home} & \textbf{Carbon Footprint} \\ \hline
\textbf{Context} & \multicolumn{4}{c|}{Motion, Phone, Room, Department, Building, Campus} & Port, Airport & Lamp, Room & Phone, Room \\ \hline
\textbf{Scenario} & \multicolumn{1}{c|}{S1} & \multicolumn{1}{c|}{S2} & \multicolumn{1}{c|}{S3} & S4 & S5 & S6 & S7 \\ \hline
\textbf{Requirement} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Query over\\ context\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Context as a\\ data source\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Opportunistic\\ Ingestion\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Policy over\\ context\end{tabular} & \begin{tabular}[c]{@{}c@{}}Distributed \\ control\end{tabular} & \begin{tabular}[c]{@{}c@{}}Data-driven \\ automation\end{tabular} & \begin{tabular}[c]{@{}c@{}}Handling data \\ heterogeneity\end{tabular} \\ \hline
\textbf{SLOC} & \multicolumn{1}{c|}{\textbf{25} (-)} & \multicolumn{1}{c|}{\textbf{19} (-)} & \multicolumn{1}{c|}{\textbf{16} (178)} & N/A & \textbf{6} (-) & \textbf{14} (45) & \textbf{8} (-) \\ \hline
\textbf{Qcx} & \multicolumn{1}{c|}{\textbf{18} (159)} & \multicolumn{1}{c|}{\textbf{6} (73)} & \multicolumn{1}{c|}{\textbf{6} (43)} & \textbf{7} (38) & \textbf{32} (-) & \textbf{11} (33) & \textbf{4} (-) \\ \hline
\end{tabular}
\caption{\textbf{Comparison of the ease-of-development and ease-of-use between \arch and baselines.} Baseline results are shown in parentheses. \textbf{SLOC:} total lines of source code and configurations required to implement components for each scenario. \textbf{Qcx:} total query complexity for completing analytics tasks in each scenario.}
\label{tab:cot}
\figspace
\figspace
\end{table*}

We report our experience using \arch to implement the apps, with a summary of results organized by app, contexts used, app scenarios, and requirements for each scenario presented in Table~\ref{tab:cot}. We highlight these requirements and how \arch meets them in each app scenario below, and include additional code examples for contexts in our Supplementary Materials.

\noindent \underline{\bf S1: Query over context.} To support querying room occupancy and energy in a smart campus, we built the device contexts and the room context in a total of 25 SLOC. The ingress and egress definitions of these contexts can be found in Table~\ref{tab:setup}. In \arch, we created four instances of the room contexts and joined the device contexts to each of them (Fig.\ref{fig:scenario}). We then ran three types of queries over the contexts: (i) querying individual context (for a room's current occupancy or energy usage), (ii) querying across multiple contexts (to rank rooms by their occupancy or energy usage), and (iii) querying across different egresses (to identify correlation between a room's energy usage and occupancy); with a total of 18 Qcx. For example, in (ii), we rank and find the least used room with:

\mintinline{shell}{> jut query kind:room@occupancy "head | sort occupancy"}

\noindent \underline{\bf S2: Context as a data source.} We developed the building context with 19 SLOC to support S2 for building-level energy and occupancy. To reuse the room-level data, we specify the room's \texttt{occupancy} and \texttt{energy} egresses in the building's ingresses. We specify ingress dataflows to aggregate the input data, \eg deriving building occupancy by dividing the number of occupied rooms by the total number rooms. We query the \texttt{BioHall@occupancy} and {@energy} for average building occupancy and energy usage, respectively, with a Qcx of 6. 

\noindent \underline{\bf S3: Opportunistic ingestion.} In the urban sensing scenario, we report network quality data using phones, laptops, and the contexts developed in S1 and S2. We configure the phone app to join/leave rooms upon detecting the change of BSSID for the WiFi AP it is currently connected to. Each time the phone changes APs, it takes a network measurement in the background using the NDT tool~\cite{ndt,ndt-ios} and reports the raw data to the context, exposed by the \texttt{phone@netTest}. We add an ingress to the room context to ingest data from \texttt{phone@netTest} in 3 SLOC, and an egress \texttt{netSpeed} that extracts download and upload bandwidth data in 5 SLOC. We repeat the same process for the laptop and its context.

\noindent \underline{\bf S4: Policy over context.} To regulate access to context data in the smart campus, we define an access control policy for campus staff and students, granting access as follows: \\
\begin{minipage}{.5\textwidth}
\minttopspace
\begin{minted}[fontsize=\footnotesize]
{yaml}
staff: ["*@netSpeed", "*@occupancy", "*@energy"]
student: ["BioLab@netSpeed", "BioLab@occupancy"]
\end{minted}
\end{minipage}

The policy allows staff to access all data in all contexts, while students are restricted to the network quality and occupancy data of the BioLab room only. Finally, we complete the smart campus app by implementing the remaining contexts for the floor, department, and campus. Overall, the implementation of the smart campus app required 92 SLOC.

\noindent \underline{\bf S5: Distributed control.} We simulate the supply chain using ship, plane, port, and airport contexts by generating join/leave events when a cargo is onboard/offboard a ship or plane, and when the ship and plane move between two ports and two airports consecutively. Each port and airport, in their apps, loads the ship or flight's joining and leaving timestamps as events to its context. We can query the \texttt{delay} egress for the delay and calculate the bottleneck of cargo latency. Note that each supply chain location has its own context and can have separate sets of access policies. Although not explicitly mentioned, such requirements for distributed control are also achieved in the previous scenarios in the smart campus. %

\noindent \underline{\bf S6: Data-driven automation.} We implement the lighting and overcrowding automation with lamps, contact and motion sensors, and reuse the room context from the smart campus app. We implement the actuation logic in the room's app with an event handler that subscribes to the occupancy egress of the room's context using the \texttt{watch()} API. If the occupancy exceeds a predefined threshold, the app sends an SMS message over the Twilio API~\cite{twilio} to alert of overcrowding. The \arch-based implementation of the automation takes a total of 14 SLOC. In the app, it takes 11 Qcx to query the room brightness and occupancy. 

\noindent \underline{\bf S7: Handling heterogeneous data.} In this last scenario, we configure the phone context to ingest and aggregate the energy readings from the rooms during its stay, by adding an ingress that ingests from \texttt{any@energy}. These data may have heterogeneous and unexpected/unknown schemas, such as data types (\eg string vs. float), names (energy'' vs. power''), or units (\eg watt'' vs. kilowatts''). For example:

\begin{minipage}{.5\textwidth}
\minttopspace
\begin{minted}[xleftmargin=0.075in,fontsize=\footnotesize]
{shell}
{watt:"80",from:"biolab",event_ts:..,ts:..}
{watt:null,from:"office",event_ts:..,ts:..}
{power:120.,unit:"watt",from:"lounge",event_ts:..,ts:..}
\end{minted}
\end{minipage}

Contexts in \arch are able to ingest these heterogeneous data records. At the phone context's ingress, we clean and convert the energy readings to the same data type and unit with:
\begin{minipage}{.5\textwidth}
\minttopspace
\begin{minted}[fontsize=\footnotesize]
{yaml}
flow: "rename watt:=power | shape(this, <{watt:float64}>) 
      | cut watt,event_ts,from"
\end{minted}
\end{minipage}

\subsection{Understanding \arch Benefits}
\label{subsec:benefit}

We repeated the implementation of S1-S7 using the two baseline frameworks, AWS IoT + Timestream (AWS) and dSpace + Postgres (dSpace). We compare the results of \arch with the baselines in Table~\ref{tab:cot}: (i) While \arch supports all scenarios, more than half of the them (4/7) cannot be easily supported by the baselines due to missing required features. (ii) Compared to the baselines, \arch simplifies the operations over context with 3x-12.2x fewer Qcx in queries, and (iii) simplifies the development of apps with 3.2x to 11.1x fewer SLOC. These benefits are a result of:

\pb{\arch simplifies the access and integration to JIT-DA data sources.} \arch handles the required coordination for adapting the data plumbing with CDG and coupler, so that developers only need to specify the sourcing intent without actually implementing the data plumbing. On the contrary, without framework support, for example, it takes 178 SLOC in AWS to support S3 (7x more than \arch), where this additional efforts include provisioning new device state tables and re-configuring the message broker~\cite{aws-iot} to append the right context information to the ingested device data. 

\pb{First-class contexts simplifies operations on context data.} In the device-oriented baseline using dSpace, device data is stored in per-device-type tables (\eg a motion sensor table) with a column indicating the room in which the device was located and the time at which the device data was ingested. For S1, it took 159 Qcx in total to implement the three queries, which is 8.8x more than \arch. This is because under the device-oriented approach, the user not only needs to filter rows in a table that belong to the room of interest but also aggregate the rows over time to derive the room occupancy values (detailed queries for this are available in our Supplementary Materials). In contrast, in \arch, context data is derived and stored in the contexts, allowing for direct query of the context data via each context's egresses. Likewise, because the context data are derived in contexts, it takes 5.4x less Qcx to specify access policies with \arch's approach, which can be specified directly over egresses. Further, when implementing S6 with dSpace, it took 3x more Qcx than \arch and 3.2x more in SLOC, with the saving from Qcx being a result of the simplification on query over context and saving from SLOC a result of removing the need to provision the device tables and access in the app.

\pb{Choice of super-structured data simplifies ingesting heterogeneous context data.} Using Zed allows data to be ingested without the need for pre-defining schemas while still being able to use the comprehensive type system in Zed to process data effectively. In comparison, we encountered difficulties when attempting S7 with the baselines: dSpace requires pre-defined tables for ingesting data; and, while AWS Timestream's dynamic schema feature automatically adds/merges new columns, this results in a wide table with sparse entries and can lead to ingestion errors when data with the same name but different types are encountered.

\pb{context provides modularity for reusing data and code while preserving distributed control.} By modularizing the data pipeline by context, contexts simplify app development by allowing apps to focus on context-oriented app logic while reusing context data of contexts. This benefit allows S2 to be completed with 12x fewer Qcx than AWS, with only 19 more SLOC required to implement the contexts. 

\subsection{Performance benchmarks}
\label{subsec:benchmark}

We aim to answer three performance-related questions for \arch: (1) How does \arch's context-oriented approach impact query performance compared to device-oriented approaches? (2) What is the overhead of using \arch for data-driven insights in the existing applications? and (3) Can \arch scale to a large number of data sources and contexts with our implementation choices? 

\begin{figure}
     \centering
     \footnotesize
     \includegraphics[width = 0.39\textwidth]{dia/query.pdf}
     \figspace
     \caption{Comparison of query latency when querying over device data (Device) vs. over context data (Context).}
     \label{fig:query}
     \figspace
\end{figure}

\pb{Impact on query performance.} To answer (1), we set up a benchmark with the smart campus app, using a week-long occupancy dataset from the UCI repository~\cite{occupancy-dataset}. We load the dataset into the motion detector contexts, which in turn populate the contexts of rooms, buildings, and the campus. We compare the latency (10 runs, reported average in $ms$) of querying the room, building, and campus occupancy using \arch and Zed lake as the baseline, as \arch already uses it as the underlying analytics engine. For \arch, we wait for the occupancy detector contexts to propagate to the other contexts, whereas for the baseline, we pre-process the dataset to add context information and then load it into Zed lake.
 
Fig.\ref{fig:query} shows that the context-oriented approach achieved an average latency of $15.8 ms$ for the room context, which is 2.2x faster than the device-oriented baseline. As the context level goes higher, the gap widens with 3.1x for the building context ($16.2 ms$ vs. $50.4 ms$) and 5.1x for the campus context ($16.2 ms$ vs. $50.4 ms$). The performance improvements stem from two factors. First, contexts contain only data ingested by the context, so querying the context directly involves loading less data compared to querying all device data, resulting in a 23\% difference in data loading time. Second, querying the context directly enables simpler queries to be evaluated compared to querying device-level data directly. Note that this improvement does not mean that \arch eliminates the need to process data, but instead shifts the processing to contexts, where the data is transformed \emph{on write/ingestion} to enable faster query evaluation. 


\begin{table}[]
\centering
\footnotesize
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Setup} & \textbf{Lamp} & \textbf{LR} & \textbf{OLR} & \textbf{OR-SMS} \\ \hline
\textbf{dSpace} & 188.84 ms & 406.91 ms & 736.01 ms & 3.02 s \\ \hline
\textbf{\arch} & 199.01 ms & 419.39 ms & 742.32 ms & 2.88 s \\ \hline
\textbf{Overhead} & 5.40 \% & 3.10\% & 0.90\% & -4.6\% \\ \hline
\end{tabular}
\caption{Overhead of integrating \arch with control applications in the existing IoT framework (dSpace). {\bf Lamp:} Automating lamp brightness. {\bf LR:} Automating room brightness. {\bf OLR:} Room brightness based on occupancy. {\bf OR-SMS:} Overcrowding alert.}
\label{tab:overhead}
\figspace
\end{table}

\pb{Integrating with existing control apps.} We compare the performance of \arch with control applications written in dSpace, which do not have a data-driven component. We reused the setup from scenario S6 (smart home, \S\ref{subsec:app}) to implement three scenarios in \arch and in dSpace. Table \ref{tab:overhead} shows that \arch adds at most 5.6\% latency overhead across the scenarios for the extra latency ($\approx 10 ms$) performing a query against the context. This querying overhead is negligible for control applications whose routines typically take several seconds, such as invoking the Twilio API to send an SMS message upon an overcrowding event. Therefore, the performance impact of \arch on control applications is insignificant.

\begin{figure}
     \centering
     \footnotesize
     \includegraphics[width = 0.37\textwidth]{dia/scale.pdf}
     \figspace
     \caption{\textbf{Scaling \arch to more contexts.} Comparing the query performance (avg. latency) with increasing number of contexts when deployed in a single-node vs. a cluster with auto-scaling enabled.}
     \label{fig:scale}
     \figspace
\end{figure}

\pb{Scale to large deployment.} \arch's target apps can have various scales from smart homes with a few rooms to buildings and campuses with hundreds of rooms. We assess whether \arch is able to handle \emph{any} of these scales. To that end, we compare the query latency with the single-node setup and a cluster setup. For the latter, we run \arch on a Kubernetes cluster running on AWS EC2 and configure a cluster autoscaler~\cite{k8s-cluster-autoscaler} to automatically provision new EC2 instances (\texttt{m5.xlarge}) under load. We run the smart campus application in S1 and S2 but now vary the number of rooms from 1 to 256; we simulate the data exchange between contexts by feeding the occupancy data to the motion sensor contexts as we did previously. As shown in Fig.\ref{fig:scale}, the results suggest that while the single-node setup can't scale beyond $\approx$60 rooms (due to the per-node resource limits on number of containers), \arch is able to scale to a much larger deployment size (256 rooms on 5 EC2 instances) with a cluster setup. 


==> prog.tex <==
\section{\arch Programming Interface}
\label{sec:prog}

\begin{table}
\footnotesize
\centering
\begin{tabular}{|l|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{API}} & \textbf{For} & \textbf{Description} \\ \hline
\textbf{sources:} [ kind:name@egress, .. ] & \cdr & Specify data sources. \\ \hline
\textbf{flow:} "operators | operators | .." & \cdr & Specify dataflow. \\ \hline
\textbf{@on.cdr}(egress="main") & \cc & Watch an egress. \\ \hline
\textbf{cdr.query}(query, egress="main") & \cc & Query an egress. \\ \hline
\textbf{cdr.load}(\{record, ..\}, egress="main") & \cc & Load data to store. \\ \hline
\textbf{cot join} [-l] name1 name2 & CLI & Join or leave \cdrs. \\ \hline
\textbf{cot query} kind:name@egress query & CLI & Query an egress. \\ \hline
\end{tabular}
\caption{\textbf{Key APIs in \arch and their usage.} \cdr: Context data router; \cc: Context controller; CLI: \arch command line.}
\label{tab:api}
\figspace
\figspace
\end{table}

We provide an overview of the programming and analytics APIs in \arch, using (simplified) examples from a smart campus app in our evaluation \S\ref{sec:eval}. Table~\ref{tab:api} summarizes the programming interfaces available in \arch.


\pb{Programming \cdr.} \arch's \cdr exposes a declarative interface built on Kubernetes~\cite{kubernetes}. This interface allows configurations to be represented as attribute-value pairs, which are stored as API objects on the Kubernetes apiserver~\cite{k8s-apiserver}. We extend this interface to support \cdr configurations, so that developers and operators can reuse existing Kubernetes tooling to handle configurations. Fig.\ref{code:building} shows the programming interface for the building BioHall. Developers or context operators can specify the ingresses and egresses on the interface, including the name, dataflow, and data sources (for ingress). Specifically, lines 4 to 16 contain the configurations for two ingresses, \texttt{room\_energy} and \texttt{room\_occupancy}, where the BioHall ingests room-level energy and occupancy as specified in the \texttt{intent} fields (lines 6 and 10) with indirect references (\S\ref{subsec:cdf}) and are resolved in the \texttt{sources} (lines 7 and 11). \arch also allows the use of an ``any'' quantifier for \cdr, as shown in Fig.\ref{code:phone-lamp} (right; line 6), which allows AlicePhone to collect energy readings from any contexts it may join. 


\begin{figure}
\footnotesize
\inputminted[xleftmargin=0.05in,numbersep=5pt,fontsize=\footnotesize]{yaml}{./code/building.yaml}
\caption{\textbf{Example \cdr configuration} for a building \cdr that generates the energy and occupancy data of BioHall.}
\label{code:building}
\figspace
\end{figure}

\begin{figure}
\centering
\footnotesize
\begin{minipage}{.21\textwidth}
\inputminted[xleftmargin=-0.05in,numbersep=4pt,fontsize=\footnotesize]{yaml}{./code/lamp.yaml}
\end{minipage}
\begin{minipage}{.25\textwidth}
\inputminted[xleftmargin=-0.1in,numbersep=4pt,fontsize=\footnotesize]{yaml}{./code/phone.yaml}
\end{minipage}
\caption{\textbf{Example \cdr configurations.} Left: A lamp \cdr and \cc. Right: A phone \cdr.}
\label{code:phone-lamp}
\figspace
\end{figure}


\begin{figure}
\footnotesize
\begin{minted}[xleftmargin=0.0in,linenos=false,]{bash}
{room_energy:80,unit:"watt",event_ts:..,ts:..}
{room_energy:120,unit:"watt",event_ts:..,ts:..}
{room_occupancy:0.5,event_ts:..,ts:..,from:"biolab1,lounge"}
{room_occupancy:1.0,event_ts:..,ts:..,from:"biolab,lounge"}
\end{minted}
\vspace{-0.1in}
\caption{Example data from building BioHall's data store, with timestamps (``event\_ts'' and ``ts'') omitted for brevity.}
\label{fig:building-records}
\figspace
\end{figure}

\pb{Processing \cdr data.} Fig.\ref{fig:building-records} shows example data records from the BioHall \cdr with the Zed data format (\S\ref{subsec:abs}). These records have different schemas and are ordered by their processing time \texttt{ts}, with the values omitted for brevity. In \arch, each data record contains two timestamps - the event timestamp (\texttt{event\_ts}) and the processing timestamp (\texttt{ts}). The event timestamp tracks when the record is generated at the data source. If the data source doesn't attach an event timestamp to the record, then the first-hop \cdr will set the \texttt{event\_ts} to be the \texttt{ts}. The \texttt{ts} on the other hand tracks when the \cdr processes the data, \ie when the ingress loads it to the store. Apart from being used in analytics such as timeseries queries, the timestamps are also used to implement exactly-once guarantees (\S\ref{subsec:runtime}).

Developers use the Zed dataflow language~\cite{zed-lang,zed-cidr} to specify the dataflow in ingresses and egresses. Zed provides convenient dataflow operators such as filtering and cleaning data using type information (\S\ref{subsec:benefit}). Note that each ingress has two attributes for dataflow specification (lines 10 to 14). The dataflow in the \texttt{flow} attribute processes data records from each data source, while the one in the \texttt{flow\_agg} attribute processes all records combined from all upstream paths (\ie the resultant data records from \texttt{flow}). Egresses are specified similarly (\eg line 19 that renames the occupancy data), except that an egress does not have \texttt{flow\_agg} nor \texttt{sources} since it reads from the \cdr's data store only.

\pb{Querying over contexts.} Users can query the egresses of \cdrs using the same dataflow language used for programming the \cdrs. For example, a building administrator can query the BioHall occupancy by running \texttt{cot query BioHall@occupancy "avg(occupancy)"}. Developers can also use the query API in \cc to run a query against the \cdr; or use the \texttt{@on.cdr(egress)} (implemented as a Python decorator) to watch and process the data streams continuously, which is useful when implementing data-driven automation. Besides, \cc can load data to the $R.store$ by calling \texttt{cdr.load({..})} with the data records, which can be used for ingesting data from sources that \arch's proxied ingestion doesn't already support, such as devices that communicate via custom device driver/libraries. For example, in Fig.\ref{code:phone-lamp}, AlicePhone may collect noise data (measured in sound-pressure-level, \emph{spl}), which are first sent to the \cc and then loaded into the \cdr. More examples of analytics using \arch are presented in \S\ref{sec:eval}. 



==> rationale.tex <==
\section{Design Goals and Approach}
\label{sec:rationale}

In this section, we elaborate on the assumptions, goals and overall approach of our work. 

\subsection{Assumptions and Problem Setup} 
Our work is motivated by the proliferation of a new generation of \emph{eclectic} data sources and their potential impact on emerging and future \emph{context-centric} applications. 

\noindent {\bf Eclectic data sources.} 
The last decade has seen an explosive growth in connected devices with 15B$+$ mobile phones~\cite{smartphone-stats} and 12.3B$+$ deployed IoT devices~\cite{iot-analytics} that are estimated to generate 
over 73.1ZB by 2025~\cite{dataprot}. These devices and their data are increasingly heterogeneous (reflecting a variety of device types and vendors), unpredictable (reflecting their association with humans and other mobile entities in the physical world), and deployed under a variety of ownership and administration models (leading to diverse configurations and policies). A recent paper~\cite{zed} refers to such data as \emph{eclectic} -  we borrow this term and extend it to the \emph{sources} of such data. Thus our focus in this paper is on eclectic data sources and their impact on application design.

\noindent {\bf Context.} 
We use the term \emph{context} to refer to the circumstances or environments in which data originate. These can be physical devices such as motion detectors and phones, as well as physical or conceptual spaces such as vehicles, rooms, and campuses. 
Contexts often - but not necessarily - exhibit the following characteristics: (i) they contain a dynamically evolving set of eclectic data sources, (ii) they are hierarchical in organization (\eg devices in a room, in a building, in a campus), (iii) a context has an ``operator'' that is distinct from its users and 
different contexts may have independent operators (\eg consider a building administrator \vs students and staff using the building). 
As a result of the above, the ownership or control over the data sources in a context is \emph{distributed} across its operators and users.

We note that, in our architecture, we choose to treat devices as simply a special form of context, which usually lies at the leaves of the context hierarchy generating (raw) data. Hence a mobile phone both belongs to its phone context and to the context of the room that it is currently in. Finally, we refer to the associations between contexts along the context hierarchy as \emph{context associations}.

\noindent {\bf Context Apps.} 
These are apps that leverage the data sources within a context so that users and operators can learn about their environment and make informed decisions regarding the same. 
A context app opportunistically consumes available input data streams, processes them, and makes them available for functions -- \eg querying, actuation -- that operate over the context. In this paper, we focus on smart-space contexts as a challenging yet important domain that is expected to grow into a \$120B$+$ market by 2026, driven by the benefits of operational efficiency, energy optimization, occupant safety, and productivity~\cite{venturebeat, markets}.
We find similar goals and constraints in other app domains such as industrial automation~\cite{boyes2018industrial,aws-iot-things-graph,cisco-iiot}, smart logistics and transportation ~\cite{samsara,cargosense,streetlight}, and urban sensing~\cite{mit-sense,citizen-science,burke2006participatory}.

Importantly, eclectic data sources are not limited to mobiles and IoT sensors. 
Consider a datacenter monitoring system: ideally, this system can ingest relevant data from a range of software and hardware components: \eg schedulers, databases, RPC stacks, switches, CPUs, GPUs, NICs, power supplies.
Each component may be developed by an independent team or vendor that uses its own approach to telemetry, alerts, profiling, and logging. Hence our monitoring system must be prepared to handle eclectic data if it is to fully leverage this rich information. More generally, as software systems have grown in complexity they increasingly adopt design paradigms---\eg microservices, API-as-a-service --- that allow systems to be designed in a distributed manner leading to greater heterogeneity and independent evolution of components. 
While we believe that CoT can serve such use cases, we leave an exploration of this to future work.

%

%




\subsection{Goals}
Our goal is to simplify and speed up the development of context apps, which is typically achieved through the use of abstraction and modularity~\cite{liskov}. This approach allows developers to reuse modular building blocks, which can hide low-level details from downstream developers, improving developer efficiency and making it easier to provide users with high-level abstractions. A rich literature on such abstractions exists for specific domains like analytics~\cite{spark,snowflake}, AI~\cite{osdi16-tensorflow,osdi18-ray}, and networking~\cite{click}, with systems identifying a minimal set of intuitive abstractions that are flexible enough to support a range of apps. Our notion of reuse also extends beyond code to data.\footnote{We point out that, for us, reuse refers not just to code but also data - \eg once computed, data for a room's context should be able for querying by a building app, a campus app, an app for emergency services, and so forth.} 

What is this minimal set of abstractions for eclectic apps? We propose an application framework whose core abstractions are based on the notion of \emph{context} -- we call this a \emph{Context of Things} framework, or \arch. Our \arch framework must support three key requirements: (i) enable by-context operations, (ii) enable opportunistic integration of eclectic data sources, (iii) support distributed control over individual data sources and contexts. Next, we provide a brief overview of how \arch achieves these goals.

\subsection{Approach}
As mentioned in \S\ref{sec:intro}, \arch achieves its goals through a combination of three key abstractions.
 {\bf Context Data Routers (CDRs)} serve as an explicit abstraction for context data. A CDR includes a templatized implementation of the CDR's ingress pipeline(s) that processes potential input data sources, a data store that holds the resultant data streams, and one or more egress views that determine how context data will be exposed to consumers. 
CDRs can be composed into a {\bf Contextualized Dataflow Graph (CDG)} that determines how the data from one context (including individual device contexts) are consumed by another. Finally, the {\bf \arch Coupler} ensures that CDRs and CDGs are automatically updated to reflect control plane events. 

This architecture meets our high level goal of simplifying context app development: developers can reuse CDRs as a modular building block while the framework takes care of common tasks such as automatically updating CDRs and CDGs in response to control events.
This approach also meets our specific requirements since: (i) CDRs offers a natural abstraction against which by-context operations can be executed, (ii) dynamic CDGs with automated runtime adaptation enables opportunistic integration of eclectic data sources, and (iii) the modular nature of CDRs allows them to be independently implemented, configured, and executed thus supporting our goal of  distributed control.

While the \arch architecture permits many deployment strategies, we anticipate that a common scenario will involve a user running a lightweight client-side app on their device that allows them to configure/query relevant CDRs that run in a cloud or on-prem deployment.  As one concrete scenario: the CDR for a user Alice's phone might be run as a service by the device vendor (Apple, Samsung) acting as \arch provider and exposed to Alice by a phone app; when Alice joins a building's context (\eg via scanning a QR code), her device CDR is automatically composed with the building's CDR; the latter might be hosted and operated by a separate \arch provider on behalf of the building owners . More constrained scenarios in which all CDRs are hosted by the same \arch provider, or an app only incorporates  users' CDRs are equally possible.


 
    



\eat{ 
\subsection{Goals}
\label{subsec:goal}

We aim to design a framework that simplifies the development and use of applications that leverage data from eclectic data sources such as mobile and IoT. Specifically, we want the framework to \emph{(i) provide modular building blocks} that allow developers to easily implement data processing logic, such as ingesting, filtering, transforming, and aggregating device-level raw data, to derive context-level data and insights that are ready to use by users and apps. The modularity of the framework should also \emph{(ii) enable the reuse of derived data across different contexts and apps.}  E.g., occupancy data of rooms can be easily reused to derive the occupancy for the building, and the building for the campus, and so on. %

To simplify the use of data apps, we want the framework to \emph{(iii) allow operations over contexts}, including querying and enforcing access policies directly over contexts. To enhance the utility and user experience of these apps, we want to enable \emph{(iv) the apps to leverage as many diverse data sources} as possible within a context, including \emph{opportunistically} consuming data from sources that may not always be available or anticipated. Further, we want to \emph{(v) reduce per-app plumbing}  for handling eclectic data sources such as data source discovery and coordinating between the app's control plane logic and data plane logic. For the latter, we want \emph{(vi) tighter integration between control and data} , where the control plane can consume and provide data from or to the data plane, while the data plane can leverage control plane signals, such as changes in context mapping, to decide when and how to process data. In particular, we want the framework to mediate and coordinate these control-data interactions \emph{without} requiring intervention from developers. Finally, we want to \emph{(vii) identify the minimal set of abstractions} required to achieve these goals within the framework. 

%
%

\subsection{Challenges}
\label{subsec:challenge}

Besides these goals, we must also tackle several unique challenges that arise in eclectic data applications.
%

\pghi{1) Distributed ownership and autonomy.} Often, the owner or ``operator'' of a context is distinct from its tenants and their devices; \eg consider a building administrator vs. the students and staff who use the building. The owners of contexts may also vary - different labs operating different rooms in a building, or different departments operating different buildings on campus. The lack of a single ownership or control across devices, apps, and contexts means that (i) an app must be prepared to discover and consume data sources in an opportunistic manner while also \emph{respecting the sources' privacy and security policies}; \eg consider a smart building app consuming data from a phone currently in the building but may not (or cannot!) continue consuming data once the phone leaves its owner . Besides, (ii) an app may consist of multiple distributed components that are operated and/or developed by multiple administrative domains, each having its own autonomy to determine how to ingest, process, and share data; \eg the smart campus app encompasses buildings, departments, rooms, and devices, following a real-world autonomy structure. Therefore, the framework should support the development and operation of apps to accommodate the distributed setup.%

\pghi{2) Dynamicity.} The binding between a data source and its context is not known a priori and can change dynamically in both time and space. For example, consider supply chain monitoring apps with devices deployed in cargo containers that travel in cargo ships and trucks between transportation facilities and warehouses; or the smart campus example with students and custodial staff carrying their personal devices and moving around campus. Hence, to perform operations over context, the app must be able to correctly identify which data streams are \emph{currently} or, depending on the app's task, \emph{was historically} associated with a context. This must be done across a range of devices, contexts, and \emph{points in time}, which can be particularly challenging when the ownership of devices and contexts differs from that of the apps. %

\pghi{3) Heterogeneity.} A consequence of distributed ownership and dynamicity is that data sources are inherently diverse in terms of both device types (\eg mobile phones, stationary sensors, mobile cameras) and their vendors. As a result, apps must be capable of consuming data from \emph{heterogeneous} and \emph{evolving} data: the schema of the data streams might not be known ahead of time, and a context may contain multiple devices that each produce data with different data schemas.

%

\subsection{Design choices}
\label{subsec:design}
%
To address the above goals and challenges, we have made three key design decisions for \arch in what follows.

\begin{figure}
     \centering
     \footnotesize
     \includegraphics[width = 0.42\textwidth]{dia/orientation.pdf}
     \caption{\textbf{Comparison of device-oriented (left) vs. context-oriented data organizations in \arch (right).} The former treats context as a label or field attached to the device data whereas \arch treats context as a first-class abstraction that can ingest, process, and store data from devices, so that the \emph{derived} context data can be directly managed and queried by users and apps.} 
     \label{fig:orientation}
     \figspace
\end{figure}

\pb{(1) First-class context.} The first design principle is to \emph{make context a first-class abstraction} in \arch through the introduction of a new data plane abstraction called \emph{context data router} (\cdr).  Each context is represented by a \cdr that can be programmed to ingest, process, store, and export/expose data for that context. This design is motivated by two key insights. First, by having the \cdr \emph{store and expose context data}---including those \emph{derived} from the ingested raw data as shown in Fig.\ref{fig:orientation}---\arch simplifies operations over context by allowing users and apps to access context data directly without combing through and translating device data. This also facilitates data reuse for other contexts and apps as they can simply use the \cdr as a data source for the context. Second, by making each context a programmable module that \emph{ingests and processes data}, we allow developers to implement modular data processing logic on a per-context basis, which can be customized and evolved independently for each context. 

We emphasize that such modularity is an important one: it allows \emph{distributing} the application logic, which typically involves a data pipeline that ingests and transforms device data to app-ready data and/or to answer app queries, into \emph{multiple modular segments} where each may be operated by a different operator, as we depict in Fig.\ref{fig:cdf}. We refer to such segment as a ``pipelet'' to contrast with data pipelines that are agnostic to the distributed structure of contexts and apps. By \emph{organizing both data and data pipeline in a distributed context-oriented manner}, \arch allows apps to preserve distributed ownership and autonomy of data management and processing for context operators, reflecting the real-world context organizations. 
%
Besides, modularizing the data pipeline by context can also simplify app development - \cdrs deal with devices and device raw data whereas apps can focus on context-oriented app logic while reusing context data of \cdrs. 

In fact, \arch goes a step further on modularity with \cdr's design. Each \cdr comprises two types of pipelets - \emph{ingress pipelets} that can ingest data and perform dataflow operations, such as data filtering and cleansing, and expressing ingestion policies for which data sources the \cdr can accept data from, and \emph{egress pipelets} that export data and  associated with egress processing logic, deciding what further data transformations should be performed over the exported data. The ingested data from the ingress pipelets is stored in the \cdr's \emph{data store} where egresses read data from.   Data in the store is typically heterogeneous and evolving due to the varying sources and processing at the ingresses. To handle this, \arch adopts the recently proposed ``super-structured'' data model called Zed~\cite{zed} to represent data in \cdr's data store and its analytics engine~\cite{zed-lake} to process/query the data in \cdrs and apps. Using Zed allows data to be ingested without the need for pre-defining schemas while still being able to use the comprehensive type system in Zed to process data efficiently and effectively. 
Finally, \cdrs are implemented with a microservice-based architecture, enabling developers and users to autonomously build and deploy/operate them. %
%

\begin{figure}
     \centering
     \footnotesize
     \includegraphics[width = 0.46\textwidth]{dia/cdf.pdf}
     \caption{\textbf{Comparison of a per-app data pipeline (top) vs. per-context data \emph{pipelets} (bottom).} The data flow between pipelets can be dynamically (re)composed to reflect context mappings. Color blocks denote ownership and autonomy boundaries.}
     \label{fig:cdf}
     \figspace
\end{figure}

\pb{(2) Contextualized data flow.} A natural follow-up question to the modular, context-oriented design mentioned above is how to \emph{compose} the \cdrs - by which we mean configuring the data flow from a \cdr's egress pipelet to another \cdr's ingress pipelet. The second design principle of \arch is to \emph{contextualize the data flow}  between \cdrs, . To achieve this, \arch introduces a new \emph{intent-based sourcing} where developers (or operators) specify the ``sourcing intent'' of which data sources an ingress can ingest data from, such as other \cdrs' egresses. The intent can be a \emph{direct reference} to specific data sources or an \emph{indirect reference} describing the desired characteristics for sources.

\arch tracks the metadata of \cdrs, including their name and egresses, and control plane signals (\eg device connections to WiFi access points, QR code scans, and user inputs), and these signals are captured by \arch's control plane to maintain context mapping (which we'll talk about shortly). At run-time,  based on the current context mapping (Fig.\ref{fig:cdf}). For example, a warehouse's \cdr that intends to ingest data from a truck will only have its sourcing intent resolve to a truck's \cdr only when the truck is in the warehouse context. By contextualizing the data flow between \cdrs, \arch allows the apps to cope with the dynamicity of real-world context mapping changes, allowing contexts to opportunistically consume data from devices , while preserving the autonomy for each context operator and app to control when and what data they want to ingest from or share with others.
%

\pb{(3) Control-data coupling.} Our last design principle is to let the framework maintain a tight coupling between the control plane and data plane. In \arch, each context has a context controller (\cc). While we introduce a new data plane abstraction for context, we let the framework, \emph{instead of the developers}, handle the coordination  between the two planes. First, the framework enforces a 1:1 mapping between a \cc and its corresponding \cdr: every time the control plane creates/deletes/updates a \cc, it correspondingly creates/deletes/updates the \cdr for that context. Besides, the framework also ensures the \cdr reacts to the control plane events as described in the previous design choice . In particular, \arch's control plane exposes a \emph{join/leave} API (based on APIs from existing IoT framework~\cite{dspace}) for users and apps to signal a device or a context's joining or leaving another context. This context mapping change is passed to the \arch's data plane to implement contextualized dataflow. This close coupling allows control actions to be explicitly and consistently reflected in the underlying data streams, making it easier for developers to ensure that changes are accurately reflected in both planes.
%
%

\subsection{Putting the pieces together: \arch overview}
\label{subsec:overview}

\begin{figure}
     \centering
     \footnotesize
     \includegraphics[width = 0.46\textwidth]{dia/arch.pdf}
     \caption{\textbf{\arch setup and architecture.} In \arch, each context has a context data router (\cdr) and a controller (\cc). \cdrs ingest, process, and store data from devices and other \cdrs while users/apps can query them for data-driven insights.}
     \label{fig:arch}
     \figspace
\end{figure}

The setup for \arch involves each facility (\eg a campus, home, retail location) having its own instance of \arch. We envision the \arch instance can be hosted on-premises, in a cloud/edge, or via a \arch SaaS provider; and the admin of the \arch instance can create accounts for context operators and apps/app users and manage access. Within the \arch instance, each context is associated with a context data router (\cdr) and a context controller (\cc). As an example, Fig.\ref{fig:arch} depicts a simplified campus \arch where the devices,\footnote{Note that devices can be considered as a special, ``bottom-level'' context. We'll explain how \arch exploits this and explain our assumptions in \S\ref{subsec:abs}.} rooms, and the building each have a \cdr and a \cc. Developers can use \arch's programming library (\S\ref{sec:prog}) to build and program new \cdrs, specifying dataflow operators and the ingestion policies (\S\ref{subsec:cdf}) for how the \cdr may ingest and process data. Besides, they can program a \cc specifying the control logic similar to what's in existing IoT frameworks~\cite{dspace}. Context operators can install \cdrs to \arch and customize their data ingestion and export policies.

At run-time, \cdrs ingest data from devices and other \cdrs; \arch adapts their data flow by deciding when a \cdr should start or stop ingesting data upon context mapping changes. Devices (their \cdrs) can be configured to \emph{join} and \emph{leave} a context based on signals such as device connections to WiFi access points, QR code scans, and user inputs and so on. An important observation is that \arch enables a bidirectional information exchange between devices and their contexts, where a device may simultaneously contribute and consume data to and from its contexts. For example, a phone running the smart campus app can report WiFi network quality data to the campus \arch; and the app can receive information from the \arch to help the user find locations with reliable network connectivity. Finally, users can interact with \arch, including discovering and querying the \cdrs, using standard user interfaces (\eg mobile apps, web browsers). We envision that other user-facing software (\eg BI tools, dashboards) can be integrated with \arch, although the design of these components is beyond the scope of this paper.

} 

==> runtime.tex <==
\section{Runtime Architecture and Execution}
\label{sec:arch}

In this section, we present the runtime components, \cdr execution, and implementation of \arch.

\subsection{\arch Runtime}
\label{subsec:runtime}

\begin{figure}
     \centering
     \footnotesize
     \includegraphics[width = 0.4\textwidth]{dia/runtime.pdf}
     \figspace
     \caption{\textbf{\arch's runtime architecture.}}
     \label{fig:runtime}
     \figspace
\end{figure}


Fig.\ref{fig:runtime} illustrates the runtime architecture of \arch, comprising the following components:

\pb{Kubernetes.} Kubernetes is a widely used container orchestrator, which \arch uses to deploys all its runtime components and uses its apiserver~\cite{k8s-apiserver}, built on etcd~\cite{etcd}, to store \cdr configurations as API objects persistently. \arch also uses the apiserver to store the groundtruth of context associations. 

\pb{\cdr and \cc.} The \cdr and \cc for a given context run in the same Kubernetes pod with one container for each. At run-time, \cdr queries and loads data from and to the Zed lake whereas \ccs may query and load data from the \cdr via the interfaces exposed by it (\S\ref{sec:prog}).

\pb{Coupler.} We implement the coupler as a Kubernetes controller that subscribes to the apiserver for context association changes and updates the \cdr's configurations (also on the apiserver). The coupler ensures the \cdr and \cc run in the same Kubernetes pod by dynamically injecting the \cc's deployment specification (from dSpace~\cite{dspace}) to the one of the \cdr upon \cdr creation. The coupler also watches registered egresses of \cdrs to update the context associations.

\pb{Zed lake.} We use the Zed lake~\cite{zed-lake} to support the data storage and querying in \arch. Zed lake stores super-structured data persistently in an object store and organizes data in ``pools'', where each pool can have multiple ``branches''. Loading data to a branch can be done atomically as a ``commit'' (achieved by a transaction journal) where one can attach metadata as part of the ``commit message''~\cite{zed-lake}. \arch leverages Zed lake by: (1) Each \cdr's data store is the ``main'' branch of a data pool. and (2) Each egress maps to its own branch named under the egress's name. 

\pb{dSpace.} dSpace is an open-source IoT framework~\cite{dspace}. \arch runs dSpace's mounter controller, which coupler invokes to handle \cc composition.



\subsection{\cdr Execution}
\label{subsec:exec}

We implement a \emph{pipelet data sync agent} that continuously pulls data from a data pool on the Zed lake, processes data with the Zed dataflow, and loads to another data pool on the Zed lake. For each egress-to-ingress pair and data-store-to-egress pair in \cdr, \arch creates an instance of pipelet agent to plumb the data flow. 

\pb{Fault-tolerance.} The pipelet agent supports exactly-once, in-order processing (EOIO) when pulling data records from one Zed lake pool/branch to another. This is achieved by writing data records along with the latest \texttt{ts} in the records (\S\ref{sec:prog}) as part of the commit message atomically, which is then stored at the target pool. Upon failure and restart, the agent will first read and cache the last-seen \texttt{ts} from the target pool's commit messages. When querying data from the source pool, the agent filters the data by reading only the ones with \texttt{ts} greater than the latest \texttt{ts}. 


\pb{Scaling the deployment.} All runtime components of \arch are run as microservices in Kubernetes~\cite{kubernetes}. \arch builds on Kubernetes's autoscaler~\cite{k8s-cluster-autoscaler} to automatically provision these components of \arch to handle large deployment. We configure the Zed lake as a Kubernetes statefulsets that can have multiple replicas backed by a load balancer, and we configure the autoscaler to use the commit rate on the Zed lake as a signal to scale up replicas for the Zed lake. Scaling down of the \arch involves redirecting \cdr requests and migrating pools, which is an ongoing work on our prototype.  %

\subsection{Implementation}
\label{subsec:impl}

Our \arch prototype consists of 2,393 SLOC of Python and 815 SLOC of Go. The \cdr programming library, code generators, the join/leave extension, and the coupler are written in Python, while the pipelet data sync agent is written in Go. Besides, we developed a Go-based CLI in $\approx$600 SLOC for \arch that includes APIs for \cdr deployment, configuration, and interaction with Zed and dSpace. To implement device connectors for proxied ingestion, we rely on vendor libraries~\cite{ios,emqx,tuyapi}, which account for $\approx$400 SLOC in Python for IoT devices and laptops, and $\approx$550 SLOC in Swift for smartphones~\cite{ios}.
